Learning from Multiway Data: Simple and Efficient Tensor Regression

Tensor regression has shown to be advantageous in learning tasks with multi-directional relatedness. Given massive multiway data, traditional methods are often too slow to operate on or suffer from memory bottleneck. In this paper, we introduce subsampled tensor projected gradient to solve the problem. Our algorithm is impressively simple and efficient. It is built upon projected gradient method with fast tensor power iterations, leveraging randomized sketching for further acceleration. Theoretical analysis shows that our algorithm converges to the correct solution in fixed number of iterations. The memory requirement grows linearly with the size of the problem. We demonstrate superior empirical performance on both multi-linear multi-task learning and spatio-temporal applications.

==> arxiv.tex <==
users such two objectives are satisfied (1) the sample size is sufficiently small (resource constraint) (2) the least square error with respect to the observation is minimized ( approximation constraint). Define a sampling operator $\Omega \in \mathbf{R}^{P \times T \times M } $, the spatio-temporal sampling problem can be defined as 
\begin{eqnarray}
\Omega & = &\argmin\limits_{(\Omega, \hat{\X}_{\Omega} )} \| I_{\Omega}\hat{\X} -  I_{\Omega}\X \| _F^2 + \lambda \|I_\Omega\|_1  \nonumber \\ 
& \text{s.t} & \text{rank}(\hat{\X}) \leq \rho
\end{eqnarray}

Where $\hat{\X}_{\Omega}$ denotes a operation of applying sampling operator $\Omega$ to $\hat{\X}$ which is a linear transformation of the vectorized tensor $\hat{\X}$.

However, the above problem is bi-convex ( convex with respect to $\Omega$ and $\hat{\X}_{\Omega}$ only separately ), it can be solved using alternating direction methods such as ADMM but the greedy algorithm might not apply (\ryedit{Need clarification} ). Therefore, we come to a second formulation for the problem. The intuition is that instead of enforcing the sparsity of the sampling operator to be sparse, we impose sparsity constraint on the resulting data tensor.
The formulation is as follows:

\begin{eqnarray}
\Omega & = &\argmin\limits_{\hat{\X}_{\Omega}} \| \hat{\X}_{\Omega} -  \X \| _{2,1}^2  \nonumber \\ 
& \text{s.t} & \text{rank}(\hat{\X}_{\Omega}) \leq \rho
\end{eqnarray}

The novelty of the above formulation compared with  \cite{bahadorifast} is that we not only impose low rank structure but also the sparsity into the objective tensor. We can also incorporate the spatial local consistency properties using the Laplacian regularizer.
% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite



%Represent the spatio-temporal data as tensor  $\X \in \R^{P \times T \times M}$ with possible side information, the spatio-temporal sampling problem  finds a tensor $\hat{\X}$ of equal dimensions, such that
%\begin{align*}
%\min_{\hat{\X} \in R(r)} & \quad  \|\hat{\X}\|_0 %\\
%\hspace{0.2in}  \mbox{ s.t.} % & 
%\quad  \|\X- \hat{\X}\|_F^2 \leq \epsilon \|\X\|_F^2 
%\end{align*}
%Where $R(r)$ denotes the space of  tensors with rank no larger than $r$. Alternatively, if we only allow the elements in the sampled tensor coming from the original full tensor, the final sampling strategy can be denoted as $\Omega \in \R^{P\ \times T \times M}$ and the problem can be formulated as 
%\begin{eqnarray}
%\label{eqn:original_problem}
%\min_{\Omega} & \quad  \|\Omega\|_0 %\\
%\hspace{0.2in}  \text{ s.t.}  \quad  \|\X- \X_\Omega\|_F^2 \leq \epsilon \|\X\|_F^2, % & 
% \quad \text{rank}(\X_\Omega) \leq r
%\end{eqnarray}
%The $L_0$ norm minimization problem is NP hard. However, sequentially sampling has shown be tractable \cite{krause2008near} provided the objective function is submodular. Therefore, we can utilize the side information and adaptively decide the next sampling entry. 


